Snaxels on a Plane

While many algorithms exist for tracing various contours for illustrating a meshed object, few algorithms organize these contours into region-bounding closed loops. Tracing closed-loop boundaries on a mesh can be problematic due to switchbacks caused by subtle surface variation, and the organization of these regions into a planar map can lead to many small region components due to imprecision and noise. This paper adapts "snaxels," an energy minimizing active contour method designed for robust mesh processing, and repurposes it to generate visual, shadow and shading contours, and a simplified visual-surface planar map, useful for stylized vector art illustration of the mesh. The snaxel active contours can also track contours as the mesh animates, and frame-to-frame correspondences between snaxels lead to a new method to convert the moving contours on a 3-D animated mesh into 2-D SVG curve animations for efficient embedding in Flash, PowerPoint and other dynamic vector art platforms.

==> snaxelframework.tex <==
\section{Snaxel framework}
Here, we describe a framework for snaxel propagation on a meshed surface. This framework can be used for segmenting mesh features~\cite{Jung:2004uf}, detecting relief on meshes~\cite{Liu:2006uu}, among a variety of other applications. Essentially the only parameter in utilizing this framework for other applications is the choice of energy function (Sec.~\ref{sec:framework:evolution}). In Sec.~\ref{sec:visualcontours}, we discuss how we use snaxels for detecting visual contours and non-photorealistic rendering. Our snaxel framework follows most closely to the methods described in \cite{Bischoff:2005va}, but also borrows ideas from \cite{Jung:2004uf,Liu:2006uu}. 


\begin{figure*}[htpb!]
\centerline{
\includegraphics[width=85mm]{fig/snaxelinfo}
\hspace{4mm}
\includegraphics[width=85mm]{fig/snaxeltopology}
}
\caption{
An example of the notation used to describe snaxels. The green circle indicates a given snaxel $s$, and the magenta and cyan circles denote the neighboring snaxels ($s_{prev}$ and $s_{next}$ respectively). The snaxel front consists of a collection of snaxels and the edges between these snaxels, which we define to always form a closed loop. Each snaxel is parameterized by the edge of the mesh that it is currently on, denoted here by ($v_{from},v_{to})$.\\
When a snaxel evolves to the end of the edge it is parameterized by, the snaxel divides. The process of division creates a new snaxel for each edge incident to the collided vertex, except for the edge the snaxel was previously on, and reconnects the front appropriately.\\
A change in topology is indicated by one snaxel colliding with another. In both cases, the colliding snaxels are removed. If the colliding snaxels are on the same front, a split occurs ({\bf top}), and a new front is created. Otherwise, if the colliding snaxels are on different fronts, the fronts are merged ({\bf bottom}).
}
\label{fig:snaxelinfo}
\end{figure*}

\subsection{Representation}
We represent snaxels as 3D points living on edges of a discrete mesh. Each snaxel is connected to two other neighboring snaxels (denoted $s_{prev}$ and $s_{next}$ for a given snaxel $s$). The linear line segments that connect neighboring snaxels are called {\it snaxel edges}.  A set of connected snaxels form a closed loop contour, which we define as a {\it snaxel front}. Figure~\ref{fig:snaxelinfo} shows an illustration of this notation.
 
A snaxel is parameterized by the edge of the mesh that it currently lies on, and its position $s_p$ is completely determined by this edge and a scalar weight in the range $[0,1]$ that defines the distance along this edge.  Borrowing notation from \cite{Bischoff:2005va}, denote vertices $v_{from}$ and $v_{to}$ as the two vertices of a given edge $e$, and $s_d$ as the scalar which interpolates between $v_{from}$ and $v_{to}$. A snaxel lying on edge $e$ has position
\begin{equation}
\label{eq:snaxelposition}
s_p = (1-s_d)v_{from} + s_dv_{to}, \ s_d \in [0,1].
\end{equation} 
Such a representation requires the edges of the mesh to be directed, but these directions can be arbitrary as long as they are consistent over time (i.e. for animations).

Snaxels that neighbor each other must always lie in the same triangle (described further in Section~\ref{sec:framework:evolution}), and thus snaxel edges will always lie on the surface of the mesh. Thus, this compact and straightforward representation is sufficient in capturing all details of a discrete surface.

\subsection{Evolution}
\label{sec:framework:evolution}
Each snaxel has an associated energy term which is defined as the sum of external energy (mesh features) as well as internal energy (features of the corresponding snaxel front). Intuitively, the external energy should be minimized when snaxels are at meaningful locations on the mesh (e.g. ridges and valleys, visual contours, etc), and the internal energy should be minimized when the snaxel front has achieved certain properties, such as smoothness, graph planarity, and so on. 

More formally, given external and internal energy functions $E_{ext}$ and $E_{int}$ respectively, we wish to find a set of snaxels $\mathbf{S}$ that minimize the following objective:
\begin{equation}
\label{eq:energyfunc}
 \underset{\mathbf{S}}{\operatorname{argmin}} \ \frac{1}{|\mathbf{S}|} \sum_{s \in \mathbf{S}} E_{int}(s) + E_{ext}(s).
\end{equation}
Depending on the choice of energy functions, this problem may be non-convex, and given our snaxel parameterization, we cannot hope to solve this optimization in closed form. However, we can find a local minimum of this function efficiently using the iterative Euler method. That is, we calculate the energy of snaxel, move the snaxel in the direction of decreasing energy, and continue to the next neighboring snaxel ($s_{next}$). This process is repeated until convergence, for each snaxel front.  Denoting $\Delta t$ as the time step and $k$ as the current iteration, the interpolating scalar $s_d$ (as defined in Eq.~\ref{eq:snaxelposition}) of snaxel $s$ on edge $e$ is updated by
\begin{equation}
s_d^{(k+1)} = s_d^{(k)} - \frac{\Delta t}{||e||} (E_{int}(s) + E_{ext}(s)),
\end{equation}
where $||e||$ is the length of the edge.
The Euler method is susceptible to numerical stability issues, and the choice of step size is crucial. Empirically, we found that $\Delta t = 0.01$ allowed for fast convergence and stable results.

As the snaxels evolve, they will collide with vertices of the mesh; equivalently, $s_d$ will lie outside of the range [0,1]. In this case, the snaxel in question $s$ will {\it divide}: a new snaxel is created for each edge incident to the collided vertex (except for the edge that the snaxel was previously on), and $s$ is removed. This process ensures that the snaxel edges lie on the surface of the mesh, and is illustrated in Fig.~\ref{fig:snaxeldivision}. Also, any excess energy in $s_d$ is passed to the newly created snaxels. For example, if $s_d = 1.4$ prior to the divide, then each newly created snaxel $s'$ will be initialized with  $s'_d = 0.4$.

\subsection{Topology control}
As the snaxel fronts move across a mesh, two types of topological events may occur: self intersection and front-front collision. These events occur when snaxels collide, and the type of event is decided by whether the snaxels are part of the same front or not. Detecting these collisions is straightforward and efficient. Both snaxels must lie on the same edge for a collision to occur, and their distance values $s_d$ must cross each other from one iteration to the next. We describe below the types of topological events and how our framework handles them.

$\bullet$ {\it Splitting} occurs at self intersection events, i.e. when two snaxels on the same front collide. In this case, the two snaxels involved in the collision are deleted, and their neighboring snaxels are joined in such a way that two new, closed loop snaxel fronts are formed.
  
$\bullet$ {\it Merging} occurs when snaxels from two different fronts collide. The two snaxels that collided are deleted, and their neighboring snaxels are joined so that the two fronts that these snaxels belonged to are connected so that one snaxel front remains.

Fig.~\ref{fig:snaxeltopology} illustrates these two topological events and how the snaxel framework handles each case.

\subsection{Implementation details}
\label{sec:snaxels:implementation}
Each snaxel front is implemented as a doubly-linked list for efficient insertion and deletion of snaxels. This is important as insertion and deletion events happen quite frequently during snaxel evolution. Below, the procedures for initializing snaxel fronts (prior to evolution) and detecting and removing degenerate snaxels are discussed.

{\bf Initializing fronts}. Snaxel fronts can be initialized in many different ways. We initialize fronts automatically by testing a conditional for each vertex of a mesh, and if the condition passes, then a front is initialized around the vertex; snaxels are placed on each edge incident to the vertex. For example, this condition could be whether or not the vertex's normal $N$ is roughly parallel to the view vector $V$ (i.e. $|N\cdot V| > \alpha$, some threshold $\alpha$). This condition should be determined based on the target application and internal and external energy functions.

{\bf Invalid snaxels}. As snaxels evolve to find minima of the energy function, several degeneracies may occur. For example, two neighboring snaxels (e.g. $s$ and $s_{next}$) should never exist on the same edge, and should be either merged or one should be deleted. Intuitively, this is problematic because both snaxels are headed in the same direction from roughly the same location, and can be considered identical snaxels. Also, if three consecutive snaxels (e.g. $s_{prev}$, $s$, and $s_{next}$) exist on a each edge of a mesh triangle, the middle snaxel ($s$) should be deleted. By a similar argument as above, the $s$ will be heading to the same vertex as either $s_{prev}$ or $s_{next}$, and can be considered degenerate. We also consider snaxel fronts of size less than three to be invalid, as we expect each front to be a closed loop. Thus, a front is deleted if the number of snaxels on it is less than three.

\begin{figure*}[htpb!]
\centerline{
\includegraphics[width=35mm]{fig/snaxelsVC/1.png}
\includegraphics[width=35mm]{fig/snaxelsVC/2.png}
\includegraphics[width=35mm]{fig/snaxelsVC/3.png}
\includegraphics[width=35mm]{fig/snaxelsVC/4.png}
\includegraphics[width=35mm]{fig/snaxelsVC/5.png}
}
\vspace{-1.5mm}
\Large \begin{tabular*}{164mm}{@{\extracolsep{\fill}}ccccc} \hspace{16mm}(a) & (b) & (c) & (d) & (e)  \end{tabular*}
\caption{Demonstration of snaxel front evolution into a visual contour.
A snaxel front (red curve) is initialized (a) and evolves according to
the energy function in Eq.~\ref{eq:vcenergy}. A topological
event occurs between (c) and (d) that splits single front into two fronts.}
\label{fig:torusExample}
\end{figure*}

\begin{figure*}
\centerline{
\includegraphics[width=35mm]{fig/snaxelsVC/6.png}
\includegraphics[width=35mm]{fig/snaxelsVC/7.png}
\includegraphics[width=35mm]{fig/snaxelsVC/8.png}
\includegraphics[width=35mm]{fig/snaxelsVC/9.png}
\includegraphics[width=35mm]{fig/snaxelsVC/10.png}
}
\Large \begin{tabular*}{164mm}{@{\extracolsep{\fill}}ccccc} \hspace{16mm}(a) & (b) & (c) & (d) & (e) \end{tabular*}
\caption{As the viewpoint changes, the snaxels move accordingly to identify the
new visual contours. Our method is robust to meshes with complex visual events,
and captures all visual contours, even those that are occluded (rendered as
dashed lines).}
\label{fig:teapotExample}
\end{figure*}


